Scattering Networks for Hybrid Representation Learning

Scattering networks are a class of designed Convolutional Neural Networks (CNNs) with fixed weights. We argue they can serve as generic representations for modelling images. In particular, by working in scattering space, we achieve competitive results both for supervised and unsupervised learning tasks, while making progress towards constructing more interpretable CNNs. For supervised learning, we demonstrate that the early layers of CNNs do not necessarily need to be learned, and can be replaced with a scattering network instead. Indeed, using hybrid architectures, we achieve the best results with predefined representations to-date, while being competitive with end-to-end learned CNNs. Specifically, even applying a shallow cascade of small-windowed scattering coefficients followed by 1$\times$1-convolutions results in AlexNet accuracy on the ILSVRC2012 classification task. Moreover, by combining scattering networks with deep residual networks, we achieve a single-crop top-5 error of 11.4% on ILSVRC2012. Also, we show they can yield excellent performance in the small sample regime on CIFAR-10 and STL-10 datasets, exceeding their end-to-end counterparts, through their ability to incorporate geometrical priors. For unsupervised learning, scattering coefficients can be a competitive representation that permits image recovery. We use this fact to train hybrid GANs to generate images. Finally, we empirically analyze several properties related to stability and reconstruction of images from scattering coefficients.

==> caltech101.tex <==

We study briefly the property of our SLE descriptor with spatial window size $16^2$, without any ad-hock spatial localization component, such Spatial Pyramid Poolin. Caltech101 is a simple dataset constituted by 9144 samples, and 102 classes. We followed the standard procedure\cite{} with 10 folds and studies the per class accuracy, with 30 training samples per class, using a linear SVM. Applying our raw scattering network leads to an accuracy of $62.8\pm0.7$, and the outputs features from $F_1,F_2,F_3$ brings respectively an absolute improvement of $13.7,17.3,20.1$ respectively as suggested in \cite{oyallon,fergus}. The accuracy of our SLE descriptor is thus $82.9\pm0.4$, which is about the same level as \ref{fergus}. However, the receptive field of \cite{fergus} is quite larger, which means the CNN is likely to build invariance to translation larger than $16$. More work to understand the properties of the SLE descriptor is needed, as its locality makes it an ideal candidate for task such image retrievial, however this is outside the scope of this paper. For the sake of comparison, we find the scattering transform combined with a ResNet-10, and followed by an averaging and a linear SVM achieves 87.7 on Caltech-101.

